Unsupervised Co-part Segmentation through Assembly

Co-part segmentation is an important problem in computer vision for its rich applications. We propose an unsupervised learning approach for co-part segmentation from images. For the training stage, we leverage motion information embedded in videos and explicitly extract latent representations to segment meaningful object parts. More importantly, we introduce a dual procedure of part-assembly to form a closed loop with part-segmentation, enabling an effective self-supervision. We demonstrate the effectiveness of our approach with a host of extensive experiments, ranging from human bodies, hands, quadruped, and robot arms. We show that our approach can achieve meaningful and compact part segmentation, outperforming state-of-the-art approaches on diverse benchmarks.

==> content/z_3_model.tex <==



\subsection{Model}\label{sec:model}

Given an image $I$, We train a network to predict the segmentation $M$,as in Fig.~\ref{fig:overview}.
The Definition of each module is in the following.

\subsubsection*{Encoder}
Given an image I, the Encoder predicts the feature V and transformation T
\begin{equation}
{\rm{E(I)  = \{ (}}{{ V}_{0}}{,}{{T}_{^{_0}}}{),(}{{ V}_1}{\rm{, }}{{T}_1}{)},...{(}{{ V}_k}{,}{{T}_k}{)}\} \label{encoder}
\end{equation}
%or represent as
%\begin{equation}{\rm{E} {(I) = \{ {V},{T}}}\} \end{equation}
%\begin{equation}{ V} = \{ {{ V}_{0}}{,}{{ V}_1}{,}...{{ V}_k}\} %\end{equation}
%\begin{equation}{T} = \{ {{T}_{0}}{,}{{T}_1}{,}...{{T}_k}\} \end{equation}

we assume V come from latent ${{{V_{lat}}}}$ by transformation matrix 
T, the transformation includes translation $t$,rotation $\theta$ and scale $s$. (now we predict $cos(\theta) $ and $sin(\theta)$
\begin{equation}
{{V  =  T( V_{lat})}}
\end{equation} 
\begin{equation}
{{V_{lat}  =  T^{-1}( V)}}
\label{latent}
\end{equation} 

\subsection{Decoder}
Given a feature ${{ V}_i}$, the decoder predicts the part scalar ${\rm{d}}_i$ that specifies relative inverse depth (i.e larger for foreground objects and image information ${{P}}_i$
\begin{equation}
{\rm{D}}({{ V}_i}{{)  =  (}}{{{d}}_i},{{P}}_i)
\end{equation}
we apply a softmax across the ${{d}}_i$  at each pixel to generate a visibility mask for each part.
\begin{equation} M= soft{\max _k}({{d)}}\end{equation}
the final output $\widetilde I$
\begin{equation}
\widetilde I = \sum\limits_{i = 1}^k {{M_i}{P_i}} 
\end{equation}
\subsection{Training process}
As shown in Fig.~\ref{sturcture_overview}.
Given two images $I^s$ and $I^t$, the encoder predicts $(V^s,T^s)$ and $(V^t,T^t)$ respectively, we  can get  $V^{s}_{lat}$ with $(V^s,T^s)$ by equation \eqref{latent}.
We assume the source and target images image share the same latent feature, so 
\begin{equation}
\widetilde V^t = {T^{^t}}V_{lat}^s
\end{equation}
We employ {\rm{D}} to reconstructs the target frame by transforming the source frame features according to the affine transformation,
so feed $\widetilde V^t$ to decoder ${\rm{D}}$, we can obtain the final predict image
${\widetilde I^t}$,$\widetilde M^t$.
For any input $I^s$, we can obtain the same output ${\widetilde I^t}$, therefore, it forces the network to learn the same latent feature $V^{s}_{lat}$.




==> geo_occlusion.tex <==
\begin{figure}[t]

   \newcommand{\formattedgraphics}[1]{\includegraphics[width=0.23\columnwidth]{#1}}
    \formattedgraphics{figures/geo_data/image_index_101.png}
    \formattedgraphics{figures/geo_data/image_index_101_part_1.png}
    \formattedgraphics{figures/geo_data/image_index_101_part_2.png}
    \formattedgraphics{figures/geo_data/image_index_101_part_3.png}
    \\
    \formattedgraphics{figures/geo_data/image_index_77.png}
    \formattedgraphics{figures/geo_data/image_index_77_part_1.png}
    \formattedgraphics{figures/geo_data/image_index_77_part_2.png}
    \formattedgraphics{figures/geo_data/image_index_77_part_3.png}
    \\ 
    \formattedgraphics{figures/geo_data/image_index_29.png}
    \formattedgraphics{figures/geo_data/image_index_29_part_1.png}
    \formattedgraphics{figures/geo_data/image_index_29_part_2.png}
    \formattedgraphics{figures/geo_data/image_index_29_part_3.png}
    
    \caption{Even the circle and  rectangle were occluded, our method can still get full shape in P from decoder.}

    \label{fig:geo}
\end{figure}



==> rebuttal_two_dance.tex <==
\begin{figure*}[h]
\vskip -0.1in
\centering
   \newcommand{\formattedgraphics}[1]{\includegraphics[width=0.16\textwidth]{#1}}
   
    \formattedgraphics{figures/rebuttal_view/1.png}
    \formattedgraphics{figures/rebuttal_view/2.png}
    \formattedgraphics{figures/rebuttal_view/3.png}
    \formattedgraphics{figures/rebuttal_view/4.png}
    \formattedgraphics{figures/rebuttal_view/5.png}
    \formattedgraphics{figures/rebuttal_view/6.png}\\
    
    \vspace{-2mm}
    \caption{Visual results of two people.}
    \label{fig:rebuttal_two_dance}
\vskip -0.1in
\end{figure*}



==> rebuttal_view.tex <==
\vspace{-0.25cm}
\begin{figure*}[h]
\centering
   \newcommand{\formattedgraphics}[1]{\includegraphics[width=0.14\textwidth]{#1}}
    \formattedgraphics{figures/rebuttal_view/p2_0.png}
    \formattedgraphics{figures/rebuttal_view/p2_1.png}
    \formattedgraphics{figures/rebuttal_view/p5_0.png}
    \formattedgraphics{figures/rebuttal_view/p5_1.png}
    \formattedgraphics{figures/rebuttal_view/p3_0.png}
    \formattedgraphics{figures/rebuttal_view/p3_1.png}\\
    \formattedgraphics{figures/rebuttal_view/f2_0.png}
    \formattedgraphics{figures/rebuttal_view/f2_1.png}
    \formattedgraphics{figures/rebuttal_view/f5_2.png}
    \formattedgraphics{figures/rebuttal_view/f5_1.png}
    \formattedgraphics{figures/rebuttal_view/f6_0.png}
    \formattedgraphics{figures/rebuttal_view/f6_1.png}\\
    \formattedgraphics{figures/rebuttal_view/1.png}
    \formattedgraphics{figures/rebuttal_view/2.png}
    \formattedgraphics{figures/rebuttal_view/3.png}
    \formattedgraphics{figures/rebuttal_view/4.png}
    \formattedgraphics{figures/rebuttal_view/5.png}
    \formattedgraphics{figures/rebuttal_view/6.png}\\
    \vspace{-2mm}
    \caption{\textbf{Top, Middle}: Visual results of applying models trained on Tai-Chi-HD (top) and VoxCeleb (middle) to videos from YouTube.
    \textbf{Bottom}: Visual results of the model trained on a video with multiple characters.} 
    \label{fig:rebuttal_generalization}
\end{figure*}
\vspace{-0.3cm}



==> vis_matrix.tex <==
\begin{figure*}[t]
    \centering
   \newcommand{\formattedgraphics}[1]{\includegraphics[width=0.95\textwidth]{#1}}
    \formattedgraphics{figures/hand_vis_rotation_and_translation/handro1.png}\\
    %\formattedgraphics{figures/hand_vis_rotation_and_translation/0057_rotation_image.png}\\
    \formattedgraphics{figures/hand_vis_rotation_and_translation/handro2.png}\\
    \caption{Visual result for mean and covariance of part mask $M_k$. The mean, represented by the black dots, are approximate with each part's center of mass; while, two columns of covariance matrix, represented by red and blue arrows, are aligned with part principal axis.\libin{To Do. R and t}}
    \label{fig:hand_matrix}
    \vspace{-4mm}
\end{figure*}



==> vis_translation.tex <==
\begin{figure*}[ht]
    \centering
   \newcommand{\formattedgraphics}[1]{\includegraphics[width=0.95\textwidth]{#1}}
   
   
    \formattedgraphics{figures/hand_vis_rotation_and_translation/0011_shift_image.png}\\
    %\formattedgraphics{figures/hand_vis_rotation_and_translation/0057_shift_image.png}\\
    \formattedgraphics{figures/hand_vis_rotation_and_translation/0080_shift_image.png}\\
    \caption{Visual result for each part's translation and covariance.}
    \label{fig:hand_shift}
\end{figure*}



==> vox_evaluation.tex <==
\begin{table}[t]
\caption{landmark regression and IoU on Voxceleb }
\label{Vox}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccr}
\toprule
measures & SCOPS & MCPS   & Ours  \\
\midrule
landmark   & 663.04 & 424.96 & 338.98\\
IoU  & 0.5045 & 0.9135 & 0.9270\\

\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}


==> x_acknowledgements.tex <==
\section*{Acknowledgements}

\textbf{Do not} include acknowledgements in the initial version of
the paper submitted for blind review.

If a paper is accepted, the final camera-ready version can (and
probably should) include acknowledgements. In this case, please
place such acknowledgements in an unnumbered section at the
end of the paper. Typically, this will include thanks to reviewers
who gave useful comments, to colleagues who contributed to the ideas,
and to funding agencies and corporate sponsors that provided financial
support.

==> z_description_of_network.tex <==
Encoder
Input image size is (H,W)
Through the two  down-sampling blocks and Hourglass\cite{newell2016hourglass}, we get feature with size ${H'\times{}W'}$ .From this feature, we use get K feature maps V and transformation T.
Decoder
The Decoder we use one residual blocks\cite{he2016resnet} and two up-sampling blocks. The size of output is ${4 \times H'\times{}W'}$, one for depth map and three for part image.
